The Communication Complexity of Optimization

We consider the communication complexity of a number of distributed optimization problems. We start with the problem of solving a linear system. Suppose there is a coordinator together with $s$ servers $P_1, \ldots, P_s$, the $i$-th of which holds a subset $A^{(i)} x = b^{(i)}$ of $n_i$ constraints of a linear system in $d$ variables, and the coordinator would like to output $x \in \mathbb{R}^d$ for which $A^{(i)} x = b^{(i)}$ for $i = 1, \ldots, s$. We assume each coefficient of each constraint is specified using $L$ bits. We first resolve the randomized and deterministic communication complexity in the point-to-point model of communication, showing it is $\tilde{\Theta}(d^2L + sd)$ and $\tilde{\Theta}(sd^2L)$, respectively. We obtain similar results for the blackboard model. When there is no solution to the linear system, a natural alternative is to find the solution minimizing the $\ell_p$ loss. While this problem has been studied, we give improved upper or lower bounds for every value of $p \ge 1$. One takeaway message is that sampling and sketching techniques, which are commonly used in earlier work on distributed optimization, are neither optimal in the dependence on $d$ nor on the dependence on the approximation $\epsilon$, thus motivating new techniques from optimization to solve these problems. Towards this end, we consider the communication complexity of optimization tasks which generalize linear systems. For linear programming, we first resolve the communication complexity when $d$ is constant, showing it is $\tilde{\Theta}(sL)$ in the point-to-point model. For general $d$ and in the point-to-point model, we show an $\tilde{O}(sd^3 L)$ upper bound and an $\tilde{\Omega}(d^2 L + sd)$ lower bound. We also show if one perturbs the coefficients randomly by numbers as small as $2^{-\Theta(L)}$, then the upper bound is $\tilde{O}(sd^2 L) + \textrm{poly}(dL)$.

==> leveragescore_lb.tex <==
% !TEX root = main.tex
\section{Missing Details in Section \ref{sec:l1regression}} \label{sec:ls_lb}
\begin{comment}
\subsection{Missing Details for Theorem \ref{thm:l1alg1} and Theorem \ref{thm:l1alg2}}\label{sec:l1bitcomplexity}
In this section, we explain why we can assume the bit complexity of all entries in the solution vector $x$ is upper bounded by $\widetilde{O}(dL)$.
We prove a more general result.
Consider an $\ell_1$-regression instance $\min_x \|Ax-b\|_1$. Suppose all entries in $A$ and $b$ are integers between $-2^{L}$ and $2^L$, then exists at least one optimal solution $x$ such that the bit complexity of all entries in $x$ is upper bounded by $\widetilde{O}(dL)$.

We may represent an $\ell_1$-regression instance as the following linear programming: 
\begin{align}
\textnormal{minimize } & \sum_{i=1}^{n} y_i && \notag \\
\textnormal{subject to } 
&  \langle A^i, x \rangle - b^i \le y_i,\label{equ:l11}\\
&  \langle A^i, x \rangle - b^i \ge -y_i \label{equ:l12}.
\end{align}

There exists an optimal solution $(x, y)$ which is a vertex of the polyhedron described above.
According to polyhedral theory, $(x, y)$ is the unique solution of a non-singular linear system with $n + d$ linear equalities, obtained by choosing $n + d$ linear inequalities in (\ref{equ:l11}) and (\ref{equ:l12}) and making them equalities. 

By the pigeonhole principle, we can find $i_1, i_2, \ldots, i_d$ such that 
$\langle A^{i_j}, x \rangle - b^{i_j} = y_{i_j}$
and
$\langle A^{i_j}, x \rangle - b^{i_j} = -y_{i_j}$,
for all $1 \le j \le d$,
which implies $\langle A^{i_j}, x \rangle = b^{i_j}$.

Let $\widetilde{A} = [(A^{i_1})^T ~(A^{i_2})^T~\ldots~(A^{i_d})^T]^T$ and $\widetilde{b} = [(b^{i_1})^T ~(b^{i_2})^T~\ldots~(b^{i_d})^T]^T$.
$x$ is the unique solution of $\widetilde{A} x =\widetilde{b}$.
Thus, by Cramer's rule, each entry of $x$ is a fraction whose numerator and denominator are integers between $-d!2^{dL}$ and $d!2^{dL}$, and thus can be represented by using at most $\widetilde{O}(dL)$ bits.
\end{comment}
%\subsection{Missing Details for Lemma \ref{lem:lewis}}\label{sec:ls_lb}


==> seidel.tex <==
\section{Seidel's algorithm}\label{sec:seidel}
We give alternative constant dimensional linear programming algorithms in both the coordinator and blackboard models based on Seidel's classical algorithm \cite{seidel1990linear}, though we need a little care on how to count the number of times we need to recompute the optimum. The different servers may have a different number of constraints so if we choose a server randomly and walk through its constraints randomly, if one server has only one constraint, that constraint will be the last one with probability $1/s$, which biases the distribution since that may be the optimal constraint, so, e.g., na\"ively with probability $d/s$ rather than $d/n$ we need to recompute the optimum, which would give expected communication $s \cdot (nd/s) = \Omega(n)$, which is too large. 

But we can randomly order constraints on each server and randomly walk through servers: suppose we are processing the $i$-th constraint in this ordering, and suppose this sits on the $j$-th server in our random ordering. Since the optimum is defined by $d$ constraints, and the servers were ordered randomly, the probability the optimum so far is on our server is at most $d/s$. Given that it is on our server, the expected number of recomputations it causes is $O(d)$, by standard Seidel analysis for a single server. So the total expected number of recomputations is $s \cdot O(d/s) \cdot d = O(d^2) = O(1)$. 

Each recomputation involves sending the current violated constraint to everyone, projecting points onto this hyperplane, and recursively solving a $(d-1)$-dimensional LP problem. We can assume everyone knows the objective $c$, since this takes $O(sL)$ communication in the coordinator model and $O(L)$ communication in the blackboard model. In the base case when recomputing the optimum in $2$ dimensions, everyone projects its constraints onto the violated constraint, and optimizes c along this line. To do so, everyone locally computes its leftmost and rightmost points along the line. We can randomly walk through the players to figure out the leftmost overall and rightmost overall point. In the blackboard model, since we are randomly walking through players, these points only get updated $O(\log s)$ times, so $O(s + L \log s)$ communication. In the coordinator model, we can transmit everything with $O(sL)$ communication. Since $d$ is constant, the bit complexity remains $O(L)$, and the number of recursive calls is $O(1)$.

\begin{theorem}\label{thm:seidel}
Seidel's algorithm can be used to solve linear programs in constant dimension with $O(sL)$ communication in the coordinator model and $O(s+L\log s)$ communication in the blackboard model.
\end{theorem}

